Extension of the Poltyrev Bound to Binary Memoryless Symmetric Channels

The Poltyrev bound provides a very tight upper bound on the decoding error probability when using binary linear codes for transmission over the binary symmetric channel and the additive white Gaussian noise channel, making use of the code's weight spectrum. In the present work, the bound is extended to memoryless symmetric channels with a discrete output alphabet. The derived bound is demonstrated on a hybrid BSC-BEC channel. Additionally, a reduced-complexity bound is introduced at the cost of some loss in tightness.

==> defs.tex <==
% TeX Defs

% The IEEEI style package
%\usepackage{spconf}

\usepackage[tbtags]{amsmath} % defines many math commands and
% \usepackage{commath}
                 % subequations environment, etc
\usepackage{amssymb}  % get, among others, blackboard bold fonts
                      % defines extra symbols like \gtreqless, etc
\usepackage{verbatim} % get comment environment, + new verbatim
\usepackage{amsxtra}  % get, eg, \accentedsymbol
%\usepackage{spacing}
\usepackage{comment}

% Includes harpoons
\usepackage{mathabx}

\usepackage{enumerate}
%\usepackage{enumitem}

\usepackage{amsfonts}
\usepackage{color}

%%% For subfigures
\usepackage{subfig}
\usepackage{caption}
%\usepackage{subcaption}

% For \smiley
\usepackage{wasysym}


%% Squeeze and order citations
\usepackage{cite}


% % Number only equations which are referred to in text
% \usepackage{mathtools}
% \mathtoolsset{showonlyrefs=true}
% % \mathtoolsset{showonlyrefs=false}

% THEOREM ENVIRONMENTS

\usepackage{amsthm}

% \theoremstyle{theorem}
\newtheorem{thm}{Theorem}%[section]
\newtheorem{lem}{Lemma}%[section]
\newtheorem{claim}{Claim}%[section]
\newtheorem{assert}{Assertion}%[section]
\newtheorem{cor}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]

\theoremstyle{definition}
\newtheorem{defn}{Definition}%[section]
\newtheorem*{defn*}{Definition}
\newtheorem{scheme}{Scheme}%[section]
\newtheorem*{scheme*}{Scheme}
\newtheorem{example}{Example}%[section]
\newtheorem{algo}{Algorithm}%[section]

\theoremstyle{remark}
\newtheorem{remark}{Remark}%[section]


\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{fdsymbol}
\newcommand{\indep}{\upvDash}
\newcommand{\dep}{\nupvDash}

\usepackage{tikz}
\usetikzlibrary{shapes,arrows,decorations.markings,positioning,calc}

\tikzstyle{plant} = [draw, fill=red!5, rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{block} = [draw, fill=blue!5, rectangle, 
    minimum height=3em, minimum width=18mm]
\tikzstyle{sum} = [draw, fill=yellow!10, circle, node distance=1cm]
\tikzstyle{coord} = [coordinate]
\tikzstyle{gain} = [draw, fill=red!5, regular polygon, regular polygon sides=3, shape border rotate=-90]
\tikzstyle{pinstyle} = [pin edge={to-,thick,black}]

\tikzstyle{BitPipe} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]

% Fits dotted rectangles around a group of blocks
\usetikzlibrary{fit,backgrounds}

%% For URLs (links) etc.
\usepackage{hyperref}
% \usepackage{url}

\usepackage{epsfig, graphicx, psfrag}

%%%%%%%\usepackage{appendix}
%%%%%%%

\usepackage[mathcal]{euscript}
% Mathcal lower-case lettters
% \newenvironment{frcseries}{\fontfamily{frc}\selectfont}{}
% \newcommand{\textfrc}[1]{{\frcseries#1}}
% % \newcommand{\mathfrc}[1]{\text{\textfrc{#1}}}
% \newcommand{\mathfrc}[1]{\mbox{\frcshape #1}}
% \providecommand{\Ber}{\mB\textfrc{er}}
\usepackage[cal=boondox]{mathalfa}
\providecommand{\Ber}{\mathcal{Ber}}
\providecommand{\Ber}{\mathcal{Bin}}

%Change maximal number of matrix columns (default = 10)
\setcounter{MaxMatrixCols}{12}

%------------------------%
% Flags for Bibliography %
%------------------------%
% \renewcommand{\davidsstar}{*}
\newcommand{\khina}{A.~Khina}
\newcommand{\invited}{}
% \newcommand{\isi}[1]{\textbf{ISI citations = #1}}
% \newcommand{\isiincl}[2]{\textbf{ISI cites (incl.\ \citeConf{#2}) = #1}}
% \newcommand{\google}{\textbf{Google Scholar cites =\ }}
% \newcommand{\googleincl}[2]{\textbf{GS cites (incl.\ \citeConf{#2}) = #1}}
% \newcommand{\googleinclabs}[3]{\textbf{GS cites (incl.\ \citeConf{#2}, \citeAbs{#3}) = #1}}
\newcommand{\PI}{}
\newcommand{\Student}{}
\newcommand{\CoRes}{}
\newcommand{\MyStudent}{}

% REFERENCE ENVIRONMENTS

\providecommand{\thmref}[1]{Theorem~\ref{#1}}
\providecommand{\assertref}[1]{Assert.~\ref{#1}}
\providecommand{\exref}[1]{Ex.~\ref{#1}}
% \providecommand{\footref}[1]{Foot.~\ref{#1}}
\providecommand{\defnref}[1]{Def.~\ref{#1}}
\providecommand{\secref}[1]{Sec.~\ref{#1}}
\providecommand{\lemref}[1]{Lemma~\ref{#1}}
\providecommand{\propref}[1]{Prop.~\ref{#1}}
\providecommand{\remref}[1]{Rem.~\ref{#1}}
\providecommand{\figref}[1]{Fig.~\ref{#1}}
\providecommand{\corref}[1]{Cor.~\ref{#1}}
\providecommand{\appref}[1]{App.~\ref{#1}}
\providecommand{\assref}[1]{Assump.~\ref{#1}}
\providecommand{\claimref}[1]{Claim~\ref{#1}}
\providecommand{\itmref}[1]{{\ref{#1}.}}
\providecommand{\algoref}[1]{Alg.~\ref{#1}}
\providecommand{\schemeref}[1]{Sch.~\ref{#1}}
\providecommand{\tabref}[1]{Tab.~\ref{#1}}
%\providecommand{\ccaption}{\caption*~{Figure~\thefigure: }}


\usepackage{refcount}
\providecommand{\footref}[1]{\footnotemark[\getrefnumber{#1}]}

\newcommand{\ie}{i.e.}
\newcommand{\iid}{i.i.d.}
\newcommand{\eg}{e.g.}
\newcommand{\etc}{etc.}
\newcommand{\viz}{viz.}
\newcommand{\etal}{\emph{et al.}}
\newcommand{\cf}{cf.}

\newcommand{\argsort}{\text{argsort}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\compls}{\mathbb{C}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\ltwor}{L^2(\reals)}
\newcommand{\ltwoz}{\ell^2(\ints)}
\newcommand{\ltwow}{L^2(\Omega)}

\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\phase}{\measuredangle}


\DeclareMathOperator{\R}{Re}
\DeclareMathOperator{\I}{Im}
\DeclareMathOperator{\plog}{log^+}

\let\limsup\relax
\DeclareMathOperator*{\limsup}{\overline{lim}}
\let\liminf\relax
\DeclareMathOperator*{\liminf}{\underline{lim}}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}
\providecommand{\Exp}[1]{{\operatorname{exp} \left\{ #1 \right\}}}
\providecommand{\E}[1]{\ensuremath{\mathbb{E} \left[ #1 \right]}}
\providecommand{\CE}[2]{\ensuremath{\mathbb{E} \left[ #1 \middle| #2 \right]}}

\renewcommand{\H}[1]{\ensuremath{H \left( #1 \right)}}
\providecommand{\CH}[2]{\ensuremath{H \left( #1 \middle| #2 \right)}}
\providecommand{\h}[1]{\ensuremath{h \left( #1 \right)}}
\providecommand{\ch}[2]{\ensuremath{h \left( #1 \middle| #2 \right)}}
\providecommand{\MI}[2]{\ensuremath{I \left( #1 ; #2 \right)}}
\providecommand{\CMI}[3]{\ensuremath{I \left( #1 ; #2 \middle| #3 \right)}}


\newcommand{\bm}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\V}[1]{{\bm{#1}}}
\newcommand{\tv}[1]{\tilde{\V{#1}}}
\renewcommand{\th}{{\tilde h}}
\newcommand{\tvzl}{\tv{w}_{l-1}}
\newcommand{\SNR}{\mathrm{SNR}}
\newcommand{\ENR}{\mathrm{ENR}}
\newcommand{\tSNR}{\widetilde\SNR}
\newcommand{\oSNR}{\overline\SNR}
\newcommand{\ov}{\bar{v}}
\newcommand{\SIR}{\mathrm{SIR}}
\newcommand{\SDR}{\mathrm{SDR}}
\newcommand{\tSDR}{\widetilde\SDR}
\newcommand{\eff}{{\mathrm{eff}}}
\newcommand{\SNReff}{\SNR_\eff}
\newcommand{\SNReq}{\SNR_\mathrm{eq}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\tot}{{\mathrm{tot}}}

\newcommand{\mX}{\mathcal{X}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mF}{\mathcal{F}}
% \newcommand{\mH}{\mathcal{H}}
\newcommand{\mH}{H}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mJ}{\mathcal{J}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}

\providecommand{\hmX}{\hat{\mX}}

\newcommand{\Comment}[1]{}
\newcommand{\old}[1]{}
\newcommand{\rem}[1]{}

\newcommand{\eps}{{\epsilon}}
\newcommand{\teps}{{\tilde{\eps}}}
\newcommand{\veps}{\varepsilon}
\newcommand{\vphi}{\varphi}

\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\Det}{\mathrm{Deter}}
\newcommand{\Vlike}{\mathrm{V-like}}

\newcommand{\modD}{\: \mathrm{mod} \: \Delta}
\newcommand{\modL}{\: \mathrm{mod} \: \Lambda}
%\newcommand{\modA}{\: \mathrm{mod} \: \mA_\Delta}
\newcommand{\modA}{\modL}
\newcommand{\Neff}{{N_\textrm{eff}^\beta}}
\newcommand{\NeffG}{N_\textrm{eff,G}^\beta}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\MMSE}{{\mathrm{MMSE}}}
\newcommand{\lattice}{\mathrm{lattice}}
\newcommand{\esupport}{\{ -\delta, \delta \}}
\newcommand{\bsupport}{\{ 1 - \delta, 1 + \delta \}}
\newcommand{\Ea}[1]{E_\alpha \left[ {#1} \right]}
\newcommand{\supp}[1]{ \mathrm{Supp} \left\{ #1 \right\} }


\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}

\providecommand{\ha}{{\hat{a}}}
\providecommand{\hb}{{\hat{b}}}
\providecommand{\hc}{{\hat{c}}}
\providecommand{\hd}{{\hat{d}}}
\providecommand{\he}{{\hat{e}}}
\providecommand{\hf}{{\hat{f}}}
\providecommand{\hg}{{\hat{g}}}
\providecommand{\hh}{{\hat{h}}}
\providecommand{\hi}{{\hat{i}}}
\providecommand{\hj}{{\hat{j}}}
\providecommand{\hk}{{\hat{k}}}
\providecommand{\hl}{{\hat{l}}}
\providecommand{\hm}{{\hat{m}}}
\providecommand{\hn}{{\hat{n}}}
\providecommand{\ho}{{\hat{o}}}
\providecommand{\hp}{{\hat{p}}}
\providecommand{\hq}{{\hat{q}}}
\providecommand{\hr}{{\hat{r}}}
\providecommand{\hs}{{\hat{s}}}
\providecommand{\ht}{{\hat{t}}}
\providecommand{\hu}{{\hat{u}}}
\providecommand{\hv}{{\hat{v}}}
\providecommand{\hw}{{\hat{w}}}
\providecommand{\hx}{{\hat{x}}}
\providecommand{\hy}{{\hat{y}}}
\providecommand{\hz}{{\hat{z}}}

\providecommand{\hA}{{\hat{A}}}
\providecommand{\hB}{{\hat{B}}}
\providecommand{\hC}{{\hat{C}}}
\providecommand{\hD}{{\hat{D}}}
\providecommand{\hE}{{\hat{E}}}
\providecommand{\hF}{{\hat{F}}}
\providecommand{\hG}{{\hat{G}}}
\providecommand{\hH}{{\hat{H}}}
\providecommand{\hI}{{\hat{I}}}
\providecommand{\hJ}{{\hat{J}}}
\providecommand{\hK}{{\hat{K}}}
\providecommand{\hL}{{\hat{L}}}
\providecommand{\hM}{{\hat{M}}}
\providecommand{\hN}{{\hat{N}}}
\providecommand{\hO}{{\hat{O}}}
\providecommand{\hP}{{\hat{P}}}
\providecommand{\hQ}{{\hat{Q}}}
\providecommand{\hR}{{\hat{R}}}
\providecommand{\hS}{{\hat{S}}}
\providecommand{\hT}{{\hat{T}}}
\providecommand{\hU}{{\hat{U}}}
\providecommand{\hV}{{\hat{V}}}
\providecommand{\hW}{{\hat{W}}}
\providecommand{\hX}{{\hat{X}}}
\providecommand{\hY}{{\hat{Y}}}
\providecommand{\hZ}{{\hat{Z}}}

\newcommand{\tb}{\tilde{b}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tZ}{\tilde{Z}}
\newcommand{\tq}{\tilde q}
\newcommand{\tg}{\tilde g}
\newcommand{\tm}{{\tilde{m}}}
\newcommand{\tL}{{\tilde L}}
\newcommand{\tw}{\tilde w}
\newcommand{\tX}{\tilde X}
\newcommand{\tgamma}{\tilde \gamma}

\newcommand{\UB}{\mathrm{UB}}
\newcommand{\Ei}{\mathrm{Ei}}

\newcommand{\tA}{\tilde A}
\newcommand{\tC}{\tilde C}
\newcommand{\tDelta}{\tilde \delta}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tN}{\tilde{N}}
\newcommand{\tkappa}{\tilde{\kappa}}
\newcommand{\tn}{\tilde{n}}
\newcommand{\htP}{\hat{\tP}}
\newcommand{\htS}{\hat{\tS}}
\providecommand{\tT}{\tilde T}
\newcommand{\tD}{\tilde D}
\newcommand{\td}{\tilde d}
\newcommand{\tH}{\tilde H}
\newcommand{\tU}{\tilde U}
\newcommand{\ts}{\tilde s}
\newcommand{\bts}{\tilde \bs}
\newcommand{\btS}{\tilde \bS}
\newcommand{\tS}{\tilde S}
\newcommand{\oS}{\overline S}
\newcommand{\ty}{\tilde y}
\newcommand{\tty}{\overline{y}}
\providecommand{\tx}{\tilde x}
\providecommand{\tz}{\tilde z}
\newcommand{\tY}{\tilde Y}
\providecommand{\tU}{{\tilde U}}
\newcommand{\trho}{r} %{\lambda} %{{\underline{\rho}}}
\newcommand{\tR}{\tilde R}
\newcommand{\ta}{\tilde a}
\newcommand{\tV}{\tilde V}
\newcommand{\tr}{\tilde r}

\newcommand{\bd}{{\bm d}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bt}{{\bm t}}
\newcommand{\bs}{{\bm s}}
\newcommand{\tinyS}{{\footnotesize \bs}}
\newcommand{\tinyW}{{\footnotesize \bw}}
\newcommand{\by}{{\bm y}}
%\newcommand{\bY}{\bm Y}
\newcommand{\bS}{\text{\bm S}}
\providecommand{\htx}{\hat{\tx}}
\newcommand{\bhS}{{\bf \hat{S}}}
\newcommand{\hbS}{{\bf \hat{S}}}
\newcommand{\hbX}{{\bf \hat{X}}}

\providecommand{\hbs}{\hat{\bs}}

\newcommand{\bn}{{\bm n}}
\newcommand{\bC}{\text{\bf C}}
\newcommand{\bH}{\text{\bf H}}
\newcommand{\bI}{\text{\bf I}}
\newcommand{\bT}{\text{\bf T}}
\newcommand{\bPhi}{{\bf \Phi}}
\newcommand{\bK}{\text{\bf K}}
\providecommand{\bU}{\text{\bf U}}
\providecommand{\bV}{\text{\bf V}}
\providecommand{\tbV}{\tilde{\bV}}
\providecommand{\tbU}{\tilde{\bU}}
\providecommand{\bD}{\text{\bf D}}
\providecommand{\tbD}{\tilde{\bD}}
\providecommand{\bW}{\text{\bf W}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bR}{\mathbf{R}}
\providecommand{\tbT}{\tilde{\bT}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bx}{{\bm x}}
\providecommand{\bu}{{\bm u}}
\providecommand{\bv}{{\bm v}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bZ}{{\bf Z}}
\providecommand{\bV}{{\bf V}}
\newcommand{\bz}{{\bm z}}
\newcommand{\ba}{{\bm a}}
\newcommand{\blambda}{{\bm \lambda}}
\providecommand{\be}{{\bm e}}
\newcommand{\bw}{{\bm w}}
\newcommand{\tbw}{\tilde{\bw}}

\newcommand{\bg}{{\bm g}}
\newcommand{\bh}{{\bm h}}

% % \newcommand{\bchi}{{\bm \chi}}
% % \newcommand{\tbchi}{\tilde {\bm \chi}}
% \newcommand{\bchi}{{\mathfrc{x}}}
% \newcommand{\tbchi}{\tilde \bchi}

\newcommand{\cS}{{\mathcal S}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cN}{{\mathcal N}}

\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}

\newcommand{\Id}{\mathcal{I}_{\delta}}
%\newcommand{\Ad}{\mathcal{A}_\Delta}
\newcommand{\Ad}{\Lambda}
\newcommand{\THP}{\text{THP}}
\newcommand{\aR}{\alpha_R}
\newcommand{\aT}{\alpha_T}
\newcommand{\aMMSE}{{\alpha_\MMSE}}
\newcommand{\aRMMSE}{{\alpha_R^\MMSE}}
\newcommand{\aTMMSE}{{\alpha_T^\MMSE}}
\newcommand{\naive}{{\text{Na\"ive}}}
\newcommand{\talpha}{{\tilde \alpha}}

\providecommand{\infinity}{\infty}

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\Norm}[1]{\left\| #1 \right\|}
\newcommand{\Nu}{\mathcal{V}}
\providecommand{\ctg}{ {\rm ctg} }
\providecommand{\ctan}{ {\rm ctg} }
\providecommand{\tg}{ {\rm tg} }
\renewcommand{\tan}{ {\rm tg} }
\providecommand{\sec}{ {\rm sec} }
\providecommand{\cosec}{ {\rm cosec} }
\providecommand{\e}{{\rm e}}
\providecommand{\comment}[1]{}
\newcommand{\thetaapp}{\theta - (\alpha - \varepsilon)}
\providecommand{\norm}[1]{\Norm{#1}}
\providecommand{\Relu}[1]{\mathrm{Relu}\left(#1\right)}


\newcommand{\BC}{{\text{BC}}}
\newcommand{\MAC}{{\text{MAC}}}
\newcommand{\LPF}{{\text{LPF}}}
\newcommand{\RF}{{\text{RF}}}
\newcommand{\AF}{{\text{AF}}}
\newcommand{\DF}{{\text{DF}}}
\newcommand{\CF}{{\text{CF}}}
\providecommand{\BW}{\text{BW}}
\newcommand{\out}{{\text{out}}}
\newcommand{\inn}{{\text{in}}}
\renewcommand{\outer}{{\text{outer}}}
\newcommand{\wh}{{\text{white}}}

\newcommand{\ej}{\e^{j 2 \pi f}}

\newcommand{\beqn}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\beq}[1]{\begin{equation}\label{#1}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\inthalf}[1]{\int_{-\frac{1}{2}}^{\frac{1}{2}} #1 df}
\newcommand{\ejj}{{\mathrm{e}^{j2\pi f}}}

\providecommand{\var}[1]{{\rm Var\left( #1 \right)}}
\providecommand{\ind}{{\perp \hspace{-2.3mm} \perp}}

\newcommand{\upharpoon}{{\upharpoonleft\hspace{-0.05cm}\upharpoonright}}

\providecommand{\Ddef}{\triangleq}

\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\ML}{\mathrm{ML}}
\newcommand{\MAP}{\mathrm{MAP}}

\newcommand{\tby}{\tilde {\bm y}}
\newcommand{\tbx}{\tilde {\bm x}}
\newcommand{\tbn}{\tilde {\bm n}}
\newcommand{\tbz}{\tilde {\bm z}}
\newcommand{\tbZ}{{\tilde{ \bf Z}}}
\providecommand{\tbX}{{\tilde{ \bf X}}}
\newcommand{\btZ}{{\tilde{ \bf Z}}}
% \newcommand{\cC}{{\cal C}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cC}{{\mathcal C}}
\providecommand{\rank}{\text{rank}}
\providecommand{\diag}{\text{diag}}
\providecommand{\qqquad}{\quad \qquad}
\providecommand{\qqqquad}{\qquad \qquad}

\providecommand{\ZF}{\text{ZF}}
\providecommand{\trace}{\text{trace}}
\providecommand{\rel}{\text{rel}}
\providecommand{\half}{\frac{1}{2}}
% % \providecommand{\bfy}{{\bf y}}
% % \providecommand{\bfz}{{\bf z}}
% \providecommand{\bfy}{{\bf \mathfrc{y}}}
% \providecommand{\bfz}{{\bf \mathfrc{z}}}
% \providecommand{\bfx}{{\bf \mathfrc{x}}}
\providecommand{\common}{\text{common}}
\providecommand{\Haug}{\mH^\text{aug}}

\providecommand{\Xcoh}{\bx^\text{C}}
\providecommand{\Xdir}{\bx^\text{D}}
\providecommand{\XCOH}{X^\text{C}}
\providecommand{\XDIR}{X^\text{D}}

%%%% From ITW2012 Full-Duplex paper
\providecommand{\ZF}{\text{ZF}}
\providecommand{\trace}{\text{trace}}
\providecommand{\rel}{\text{rel}}
\providecommand{\src}{\text{t}}
\providecommand{\dst}{\text{r}}
\providecommand{\half}{\frac{1}{2}}

\providecommand{\Xcoh}{\bx^\text{C}}
\providecommand{\Xdir}{\bx^\text{D}}
\providecommand{\xdir}{x^\text{D}}
\providecommand{\xcoh}{x^\text{C}}
\providecommand{\XCOH}{X^\text{C}}
\providecommand{\XDIR}{X^\text{D}}
\providecommand{\bXCOH}{{\bf X^\text{C}}}
\providecommand{\bXDIR}{{\bf X^\text{D}}}
\providecommand{\tty}{\overline{\by}}
\providecommand{\tby}{\tilde {\bm y}}
\providecommand{\tbx}{\tilde {\bm x}}
\providecommand{\tbn}{\tilde {\bm n}}
\providecommand{\tbz}{\tilde {\bm z}}
\providecommand{\ttz}{\overline{\bz}}
\providecommand{\bfy}{{\cal Y}}
\providecommand{\bfz}{{\cal Z}}
\providecommand{\ttz}{\overline{\bz}}
\providecommand{\BdirTx}{B^\text{D}_t}
\providecommand{\BcohTx}{B^\text{C}_t}
\providecommand{\BcohRel}{B^\text{C}_\rel}
\providecommand{\equivalent}{{\text{equiv}}}

%% New parentheses sizes (similar to \bigg ane alike)
\makeatletter
\newcommand{\vast}{\bBigg@{4}}
\newcommand{\Vast}{\bBigg@{5}}
\makeatother

%%%% From ISIT2011 two-way relay paper
\providecommand{\CS}{{\text{CS}}}
\providecommand{\PNC}{{\text{PNC}}}

\newcommand{\opI}{I}
\providecommand{\causalKer}[2]{P(#1 \upupharpoons #2)}
\providecommand{\condCausalKer}[3]{P(#1 \upupharpoons #2 | #3)}
\providecommand{\MI}[2]{{\opI \left( #1 ; #2 \right)}}
\providecommand{\DI}[2]{{\opI \left( #1 \to #2 \right)}}
% \providecommand{\CDI}[3]{{\opI \left( #1 \to #2 | #3\right)}}
% \providecommand{\dsx}[1]{{\delta s_{#1}(t)}}
\providecommand{\dsx}[1]{{s'_{#1}(t)}}

\providecommand{\quant}[1]{{Q_{\Lambda} \left( #1 \right)}}


\providecommand{\KL}[2]{{\bbD \left( #1 \middle\| #2 \right)}}
\providecommand{\CMI}[3]{{\opI \left( #1 ; #2 \middle| #3 \right)}}
\providecommand{\CDI}[3]{{\opI \left( #1 \to #2 \upupharpoons #3 \right)}}
\providecommand{\CKL}[3]{{\bbD \left( #1 \middle\| #2 \middle| #3 \right)}}
\renewcommand{\H}[1]{{H \left( #1 \right)}}
\providecommand{\h}[1]{{h \left( #1 \right)}}
\providecommand{\CH}[2]{{H \left( #1 \middle| #2 \right)}}
\providecommand{\Ch}[2]{{h \left( #1 \middle| #2 \right)}}
\providecommand{\C}[1]{\text{C} \left( #1  \right)}
\newcommand{\hbg}{\hat{\bg}}
\newcommand{\hbgo}{\hat{\bg}^\perp}
\newcommand{\zg}{z_g}
\newcommand{\ug}{u_g}
\newcommand{\vg}{v_g}
\newcommand{\wg}{w_g}
\newcommand{\twg}{\tilde{w}_g}
\newcommand{\zgo}{z_{g^\perp}}

% Cluster
\providecommand{\inter}{{\text{inter}}}
\providecommand{\bHinter}{\bH_{\text{inter}}}
\providecommand{\bxinter}{\bx_{\text{inter}}}

\providecommand{\Cmac}[1]{ \cC_\MAC \left( #1 \right) } 

\providecommand{\dB}{\mathrm{dB}}
\providecommand{\self}{\textrm{self}}
\providecommand{\intra}{\textrm{intra}}
\providecommand{\inter}{\textrm{inter}}

\providecommand{\TWOD}{\text{2D}}
\providecommand{\oD}{\bar{D}}

\providecommand{\bbD}{\mathbb{D}}
\providecommand{\bbE}{\mathbb{E}}
\providecommand{\bbh}{\mathbb{h}}
\providecommand{\bbH}{\mathbb{H}}
\providecommand{\bbI}{\mathbb{I}}
\providecommand{\bbP}{\mathbb{P}}

\providecommand{\E}[1]{\bbE \left[ #1 \right]}
\providecommand{\CE}[2]{\bbE \left[ #1 \middle| #2 \right]}
\providecommand{\Esub}[2]{\bbE_{#1} \left[ #2 \right]}
\providecommand{\CEsub}[3]{\bbE_{#1} \left[ #2 \middle| #3 \right]}
\providecommand{\Pinf}{P_\infty}
\providecommand{\CP}[2]{P \left( #1 \middle| #2 \right)}

\providecommand{\packet}{F}
\providecommand{\PACKET}{a}
% \providecommand{\IF}{\mathrm{if }}
\providecommand{\IF}{}
\providecommand{\AND}{\textrm{ and }}

% \providecommand{\RDF}[2]{\cR \left( \frac{#1}{#2} \right)}
\providecommand{\RDF}[2]{\half \log \left( \frac{#1}{#2} \right)}
\providecommand{\erasure}{\davidsstar}
\providecommand{\Dweight}{D^\mathrm{Weighted}}
\providecommand{\betaut}{b}
\providecommand{\tind}{t}
\providecommand{\twopi}{\tau}

\providecommand{\indind}{k}
\providecommand{\alphat}{\alpha_\tind}
\providecommand{\alphai}{\alpha_\indind}
\providecommand{\alphapr}{\alpha_{\tind-1}}
\providecommand{\Wt}{W_\tind}
\providecommand{\Wpr}{W_{\indind-1}}
\providecommand{\Wi}{W_\indind}
\providecommand{\Rt}{R_\tind}
\providecommand{\rt}{r_\tind}
\providecommand{\Ri}{R_\indind}
\providecommand{\Rpr}{R_{\indind-1}}
\providecommand{\Rone}{R_1}
\providecommand{\Bt}{B_\tind}
\providecommand{\Npackets}{K}

\providecommand{\Eig}{\lambda}
\providecommand{\SNRf}{\SNR_\mathrm{F}}
\providecommand{\SNRb}{\SNR_\mathrm{B}}
\providecommand{\costX}{q}
\providecommand{\costU}{r}

% \renewcommand{\gamma}{\ENR}
\newcommand{\Dzz}{D_\mathrm{ZZ}}
\newcommand{\Dww}{D_\mathrm{WW}}
\providecommand{\Edsgn}{\tE}
\newcommand{\PR}[1]{\Pr\left( #1 \right)}
\newcommand{\CPR}[2]{\Pr\left( #1 \middle| #2 \right)}
\providecommand{\tsigma}{\tilde{\sigma}}
\providecommand{\Nmin}{N_{\min}}

\providecommand{\bullets}{\bullet \bullet \bullet}

\newcommand {\Rh} {R_{\mbox{\tiny h}}}
\newcommand {\Lh} {L_{\mbox{\tiny h}}}
\newcommand {\Mh} {{M_{\mbox{\tiny h}}}}

\newcommand{\dfn}{\triangleq}
\newcommand{\exe}{\doteq}
\providecommand{\dotgeq}{\dot{\geq}}
\newcommand{\gexe}{\dotgeq}

\providecommand{\Exp}[1]{\ensuremath{{\operatorname{exp} \left\{ #1
\right\}}}}

\providecommand{\dotleq}{\mathrel{\dot{\leq}}}
% \providecommand{\dotleq}{\dot{\leq}}
\providecommand{\xto}[2]{\xrightarrow[#2]{#1}}
\providecommand{\Q}[1]{\ensuremath{Q \left( #1 \right)}}

\providecommand{\lrp}[1]{\left( #1 \right)}
\providecommand{\lrr}[1]{\left( #1 \right)}
\providecommand{\lrs}[1]{\left[ #1 \right]}
\providecommand{\lrc}[1]{\left\{ #1 \right\}}

\providecommand{\IV}{V}
\providecommand{\RV}{V}
